d-wave pairing from spin fluctuations in the KxFe{2-y}Se2 superconductors

Angle-resolved photoemission spectroscopy measurements on the recently discovered superconduc- tors in the KFe2Se2 family with critical temperatures up to - 33K suggest that no Fermi pockets of hole character centered on the {\Gamma} point of the Brillouin zone are present, in contrast to all other known ferropnictide and ferrochalcogenide superconductors. Using a fluctuation exchange approximation and a 5-orbital tight-binding description of the band structure, we calculate the effective pairing interaction. We find that the pairing state in this system is most likely to have d-wave symmetry due to pair scattering between the remaining electron Fermi pockets at wave vector q - ({\pi}, {\pi}), but without any symmetry-imposed nodes for the given Fermi surface. We propose experimental tests of this result, including the form of the resonance spectrum probed by inelastic neutron scattering.

==> PaxHeader/KFeSe_v2_tam.tex <==
17 uid=287928490
20 ctime=1296011996
20 atime=1296011996
38 LIBARCHIVE.creationtime=1295980342
24 SCHILY.dev=234881026
23 SCHILY.ino=24712242
18 SCHILY.nlink=1

